Do We Really Need to Drop Items with Missing Modalities in Multimodal Recommendation?

Generally, items with missing modalities are dropped in multimodal recommendation. However, with this work, we question this procedure, highlighting that it would further damage the pipeline of any multimodal recommender system. First, we show that the lack of (some) modalities is, in fact, a widely-diffused phenomenon in multimodal recommendation. Second, we propose a pipeline that imputes missing multimodal features in recommendation by leveraging traditional imputation strategies in machine learning. Then, given the graph structure of the recommendation data, we also propose three more effective imputation solutions that leverage the item-item co-purchase graph and the multimodal similarities of co-interacted items. Our method can be plugged into any multimodal RSs in the literature working as an untrained pre-processing phase, showing (through extensive experiments) that any data pre-filtering is not only unnecessary but also harmful to the performance.

==> figures/motivation.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/motivation.pdf}
    \caption{Results of BPRMF (in blue) and VBPR (in red) on Music and Beauty datasets. Compared to the setting where items with missing modalities are dropped (top), the imputation of missing modalities (bottom) can preserve or even widen the performance gap between BPRMF and VBPR.}
    \label{fig:motivation}
\end{figure}

==> figures/pipeline.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/pipeline.pdf}
    \caption{Proposed graph-aware imputation. The steps involve (a) projection into the item-item co-interactions graph; (b) top-k sparsification; (c) normalization (Laplacian or personalized page rank); (d) missing modalities imputation.}
    \label{fig:pipeline}
\end{figure}

==> tables/datasets_old.tex <==
\begin{table*}[!t]
    \caption{Statistics of tested datasets. We report the number of items with missing \textcolor{Mahogany}{\textbf{visual}} and \textcolor{RoyalBlue}{\textbf{textual}} features, and the dataset statistics before and after dropping those items (indicated without and with the apex, respectively).}\label{tab:datasets}
    \centering
    \begin{tabular}{lrrrrr}
    \toprule
        \multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{$|\mathcal{U}|\;/\;|\mathcal{U}'|$}} & \multirow{2}{*}{\textbf{$|\mathcal{I}|\;/\;|\mathcal{I}'|$}} & \multirow{2}{*}{\textbf{$|\mathcal{R}|\;/\;|\mathcal{R}'|$}} & \multicolumn{2}{c}{\textbf{Missing}} \\ \cmidrule{5-6}
        & & & &  \textcolor{Mahogany}{Visual} & \textcolor{RoyalBlue}{Textual} \\
        \cmidrule{1-6}
        Baby & 19,445 / 19,440 & 7,050 / 6,382 & 160,792 / 138,149 & 13 & 667 \\
        Toys \& Games & 19,412 / 19,410 & 11,924 / 11,089 & 167,597 / 146,640 & 17 & 832  \\
        Beauty & 22,363 / 22,293 & 12,101 / 11,124 & 198,502 / 165,772 & 7 & 977 \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/datasets_old_old.tex <==
\begin{table*}[!t]
    \caption{Statistics of tested datasets. We report the number of items with missing \textcolor{Mahogany}{\textbf{visual}} and \textcolor{RoyalBlue}{\textbf{textual}} features, and the dataset statistics before and after dropping those items (indicated without and with the apex, respectively).}\label{tab:datasets}
    \centering
    \begin{tabular}{lrrrrr}
    \toprule
        \multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{$|\mathcal{U}|\;/\;|\mathcal{U}'|$}} & \multirow{2}{*}{\textbf{$|\mathcal{I}|\;/\;|\mathcal{I}'|$}} & \multirow{2}{*}{\textbf{$|\mathcal{R}|\;/\;|\mathcal{R}'|$}} & \multicolumn{2}{c}{\textbf{Missing}} \\ \cmidrule{5-6}
        & & & &  \textcolor{Mahogany}{Visual} & \textcolor{RoyalBlue}{Textual} \\
        \cmidrule{1-6}
        Digital Music & 5,541 / 5,349 & 3,568 / 2,453 & 64,706 / 51,516 & 2 & 1,114\\
        Office Products & 4,905 / 4,891 & 2,420 / 1,746 & 53,258 / 35,185 & 0 & 674\\ 
        Baby & 19,445 / 19,440 & 7,050 / 6,382 & 160,792 / 138,149 & 14 & 667 \\
        Toys \& Games & 19,412 / 19,410 & 11,924 / 11,089 & 167,597 / 146,640 & 19 & 832  \\
        Beauty & 22,363 / 22,293 & 12,101 / 11,124 & 198,502 / 165,772 & 7 & 977 \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/rq2_old.tex <==
\begin{table*}[!t]
\caption{}\label{tab:rq2}
    \centering
    \resizebox{0.6\textwidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Baby}} & \multicolumn{2}{c}{\textbf{Toys \& Games}} & \multicolumn{2}{c}{\textbf{Beauty}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        & Recall & nDCG & Recall & nDCG & Recall & nDCG \\ \cmidrule{1-7}
        \CC{20}BPRMF (\textsc{Base}) & \CC{20}4.56 & \CC{20}2.23 & \CC{20}8.55 & \CC{20}4.55 & \CC{20}9.43 & \CC{20}4.85 \\ \cmidrule{1-7}
        BPRMF-M (\textsc{Zeros}) & 5.03 & 2.49 & 10.07 & 5.42 & 9.80 & 5.08 \\
        BPRMF-M (\textsc{Random}) & 5.24 & 2.64 & 9.80 & 5.37 & 10.09 & 5.22 \\
        BPRMF-M (\textsc{GlobalMean}) & 4.98 & 2.46 & 9.76 & 5.33 & 10.55 & 5.55 \\
        \cmidrule{1-7}
        BPRMF-M (\textsc{NeighMean}) & 5.05 & 2.51 & 10.10 & 5.45 & 9.82 & 5.09 \\
        BPRMF-M (\textsc{PersPageRank}) \\
        BPRMF-M (\textsc{FeatProp}) & 5.71 & 2.82 & 10.37 & 5.62 & 10.83 & 5.73 \\
        \cmidrule{1-7} \textit{Improvement (\%)} \\
        \cmidrule{1-7} 
        \CC{20}NGCF (\textsc{Base}) & \CC{20}5.59 & \CC{20}2.81 & \CC{20}8.22 & \CC{20}4.23 & \CC{20}8.92 & \CC{20}4.56 \\ \cmidrule{1-7}
        NGCF-M (\textsc{Zeros}) & 6.76 & 3.39 & 8.56 & 4.38 & 9.64 & 4.99 \\
        NGCF-M (\textsc{Random}) & 6.57 & 3.30 & 8.32 & 4.31 & 9.74 & 5.01 \\
        NGCF-M (\textsc{GlobalMean}) & 6.89 & 3.50 & 8.62 & 4.39 & 9.73 & 5.02 \\
        \cmidrule{1-7}
        NGCF-M (\textsc{NeighMean}) & 7.00 & 3.57 & 8.77 & 4.48 & 10.32 & 5.35 \\
        NGCF-M (\textsc{PersPageRank}) & & &  &  \\
        NGCF-M (\textsc{FeatProp}) & 7.07 & 3.58 & inria & inria & cineca & cineca \\ \cmidrule{1-7} \textit{Improvement (\%)} \\
        \bottomrule
    \end{tabular}}
\end{table*}

==> tables/rq2_old_old.tex <==
\begin{table*}[!t]
\caption{}\label{tab:rq2}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcccccccccc}
    \toprule
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Digital Music}} & \multicolumn{2}{c}{\textbf{Office Products}} & \multicolumn{2}{c}{\textbf{Baby}} & \multicolumn{2}{c}{\textbf{Toys \& Games}} & \multicolumn{2}{c}{\textbf{Beauty}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        \cmidrule(lr){8-9}
        \cmidrule(lr){10-11}
        & Recall & nDCG & Recall & nDCG & Recall & nDCG & Recall & nDCG & Recall & nDCG \\ \cmidrule{1-11}
        \CC{20}BPRMF (\textsc{Base}) & \CC{20}24.59 & \CC{20}13.69 & \CC{20}8.51 & \CC{20}4.55 & \CC{20}4.56 & \CC{20}2.23 & \CC{20}8.55 & \CC{20}4.55 & \CC{20}9.43 & \CC{20}4.85 \\ \cmidrule{1-11}
        BPRMF-M (\textsc{Zeros}) & 24.85 & 14.02 & 9.49 & 5.24 & 5.03 & 2.49 & 10.07 & 5.42 & 9.80 & 5.08 \\
        BPRMF-M (\textsc{Random}) & 25.65 & 14.24 & 8.57 & 4.75 & 5.24 & 2.64 & 9.80 & 5.37 & 10.09 & 5.22 \\
        BPRMF-M (\textsc{GlobalMean}) & 24.81 & 14.03 & 9.46 & 5.30 & 4.98 & 2.46 & 9.76 & 5.33 & 10.55 & 5.55 \\
        \cmidrule{1-11}
        BPRMF-M (\textsc{NeighMean}) & 24.77 & 13.89 & 9.53 & 5.23 & 5.05 & 2.51 & 10.10 & 5.45 & 9.82 & 5.09 \\
        BPRMF-M (\textsc{PersPageRank}) \\
        BPRMF-M (\textsc{FeatProp}) & 26.03 & 14.56 & 10.09 & 5.41 & 5.71 & 2.82 & 10.37 & 5.62 & 10.83 & 5.73 \\
        \cmidrule{1-11} \textit{Improvement (\%)} &  &  &  &  &  &  &  &  \\
        \cmidrule{1-11} 
        \CC{20}NGCF (\textsc{Base}) & \CC{20}24.12 & \CC{20}13.06 & \CC{20}8.18 & \CC{20}3.91 & \CC{20}5.59 & \CC{20}2.81 & \CC{20}8.22 & \CC{20}4.23 & \CC{20}8.92 & \CC{20}4.56 \\ \cmidrule{1-11}
        NGCF-M (\textsc{Zeros}) & 24.14 & 13.03 & 10.55 & 5.34 & 6.76 & 3.39 & 8.56 & 4.38 & 9.64 & 4.99 \\
        NGCF-M (\textsc{Random}) & 24.42 & 13.28 & 10.44 & 5.19 & 6.57 & 3.30 & 8.32 & 4.31 & 9.74 & 5.01 \\
        NGCF-M (\textsc{GlobalMean}) & 23.99 & 13.05 & 10.69 & 5.35 & 6.89 & 3.50 & 8.62 & 4.39 & 9.73 & 5.02 \\
        \cmidrule{1-11}
        NGCF-M (\textsc{NeighMean}) & 23.86 & 12.65 & 11.33 & 5.79 & 7.00 & 3.57 & 8.77 & 4.48 & 10.32 & 5.35 \\
        NGCF-M (\textsc{PersPageRank}) & & &  &  \\
        NGCF-M (\textsc{FeatProp}) & 25.08 & 13.58 & 11.60 & 5.81 & 7.07 & 3.58 & inria & inria & cineca & cineca \\ \cmidrule{1-11} \textit{Improvement (\%)} \\\cmidrule{1-11} 
        \CC{20}LightGCN (\textsc{Base}) & \CC{20}26.61 & \CC{20}14.49 & \CC{20}11.55 & \CC{20}6.12 & \CC{20}7.36 & \CC{20}3.76 & \CC{20}10.22 & \CC{20}5.43 & \CC{20}11.61 & \CC{20}6.02 \\ \cmidrule{1-11}
        LightGCN-M (\textsc{Zeros}) & 26.75 & 14.59 & 11.69 & 6.40 & 7.71 & 3.89 & 10.44 & 5.60 & 12.02 & 6.33 \\
        LightGCN-M (\textsc{Random}) & 26.25 & 14.34 & 11.43 & 6.27 & 7.49 & 3.83 & 10.42 & 5.64 & 11.54 & 6.10\\
        LightGCN-M (\textsc{GlobalMean}) & 26.85 & 14.91 & 11.78 & 6.42 & 7.69 & 3.90 & 10.71 & 5.84 & 12.01 & 6.32 \\
        \cmidrule{1-11}
        LightGCN-M (\textsc{NeighMean}) & 27.37 & 15.21 &  12.01 & 6.69 & 7.74 & 3.92 & 11.26 & 6.06 & 12.03 & 6.32 \\
         LightGCN-M (\textsc{PersPageRank}) & & &  &  \\
        LightGCN-M (\textsc{FeatProp}) & 27.35 & 15.22 & 11.89 & 6.49 & 7.74 & 3.92 & 11.27 & 6.10 & 12.16 & 6.34 \\ \cmidrule{1-11} \textit{Improvement (\%)} \\
        \bottomrule
    \end{tabular}}
\end{table*}

==> tables/rq3_1.tex <==
\begin{table*}[!t]
\caption{}\label{tab:rq3}
    \centering
    \begin{tabular}{lcccc}
    \toprule
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Digital Music}} & \multicolumn{2}{c}{\textbf{Beauty}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Recall & nDCG & Recall & nDCG \\ \cmidrule{1-5}
        FREEDOM (\textsc{Zeros}) & 25.60 & 13.78 & 10.99 & 5.76 \\
        FREEDOM (\textsc{Random}) & 26.81 & 14.46 & 13.00 & 6.73 \\
        FREEDOM (\textsc{GlobalMean}) & 26.62 & 14.61 & 13.02 & 6.80 \\
        \cmidrule{1-5}
        FREEDOM (\textsc{NeighMean}) & 26.17 & 14.35 & 13.23 & 6.88 \\
        FREEDOM (\textsc{FeatProp}) & \underline{27.09} & \textbf{14.91} & \underline{13.26} & \underline{6.96} \\
        FREEDOM (\textsc{PersPageRank}) & \textbf{27.18} & \underline{14.88} & \textbf{13.28} & \textbf{7.00} \\
        \cmidrule{1-5}
        BM3 (\textsc{Zeros}) & 24.64 & 13.00 & 11.31 & 5.96 \\
        BM3 (\textsc{Random}) & 24.29 & 12.93 & 11.35 & 5.88  \\
        BM3 (\textsc{GlobalMean}) & 24.27 & 12.88 & 11.35 & 5.91 \\
        \cmidrule{1-5}
        BM3 (\textsc{NeighMean}) & 24.46 & 12.95 & \underline{11.48} & \underline{6.01} \\
        BM3 (\textsc{FeatProp}) & \underline{25.00} & \textbf{13.55} & \textbf{11.49} & \textbf{6.04} \\
        BM3 (\textsc{PersPageRank}) & \textbf{25.11} & \underline{13.44} & 11.35 & 5.96 \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/rq3_1_old.tex <==
\begin{table*}[!t]
\caption{}\label{tab:rq3}
    \centering
    \begin{tabular}{lcccc}
    \toprule
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Baby}} & \multicolumn{2}{c}{\textbf{Beauty}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Recall & nDCG & Recall & nDCG \\ \cmidrule{1-5}
        FREEDOM (\textsc{Zeros}) & 7.30 & 3.76 & 10.99 & 5.76 \\
        FREEDOM (\textsc{Random}) & 8.37 & 4.30 & 13.00 & 6.73 \\
        FREEDOM (\textsc{GlobalMean}) & 8.25 & 4.23 & 13.02 & 6.80 \\
        \cmidrule{1-5}
        FREEDOM (\textsc{NeighMean}) & 8.63 & 4.42 & 13.23 & 6.88 \\
        FREEDOM (\textsc{PersPageRank}) & & & cineca & cineca \\
        FREEDOM (\textsc{FeatProp}) & & & inria & inria \\
        \cmidrule{1-5}
        BM3 (\textsc{Zeros}) & 7.64 & 3.87 & 11.31 & 5.96 \\
        BM3 (\textsc{Random}) & 7.53 & 3.84 & 11.35 & 5.88  \\
        BM3 (\textsc{GlobalMean}) & 7.70 & 3.94 & 11.35 & 5.91 \\
        \cmidrule{1-5}
        BM3 (\textsc{NeighMean}) & 7.99 & 4.06 & 11.48 & 6.01 \\
        BM3 (\textsc{PersPageRank}) & & & cineca & cineca \\
        BM3 (\textsc{FeatProp}) & & & inria & inria \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/rq3_1_stars.tex <==
\begin{table*}[!t]
\caption{}\label{tab:rq3}
    \centering
    \begin{tabular}{lcccc}
    \toprule
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Digital Music}} & \multicolumn{2}{c}{\textbf{Beauty}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
        & Recall & nDCG & Recall & nDCG \\ \cmidrule{1-5}
        FREEDOM (\textsc{Zeros}) & 25.60 & 13.78 & 10.99 & 5.76 \\
        FREEDOM (\textsc{Random}) & 26.81 & 14.46 & 13.00 & 6.73 \\
        FREEDOM (\textsc{GlobalMean}) & 26.62 & 14.61 & 13.02 & 6.80 \\
        \cmidrule{1-5}
        FREEDOM (\textsc{NeighMean}) & 26.17 & 14.35 & 13.23 & 6.88 \\
        FREEDOM (\textsc{FeatProp}) & \underline{27.09} & \textbf{14.91} & \underline{13.26*} & \underline{6.96*} \\
        FREEDOM (\textsc{PersPageRank}) & \textbf{27.18} & \underline{14.88} & \textbf{13.28*} & \textbf{7.00*} \\
        \cmidrule{1-5}
        BM3 (\textsc{Zeros}) & 24.64 & 13.00 & 11.31 & 5.96 \\
        BM3 (\textsc{Random}) & 24.29 & 12.93 & 11.35 & 5.88  \\
        BM3 (\textsc{GlobalMean}) & 24.27 & 12.88 & 11.35 & 5.91 \\
        \cmidrule{1-5}
        BM3 (\textsc{NeighMean}) & 24.46 & 12.95 & \underline{11.48} & \underline{6.01} \\
        BM3 (\textsc{FeatProp}) & \underline{25.00} & \textbf{13.55} & \textbf{11.49*} & \textbf{6.04*} \\
        BM3 (\textsc{PersPageRank}) & \textbf{25.11} & \underline{13.44} & 11.35* & 5.96* \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/rq3_old.tex <==
\begin{table*}[!t]
\caption{}\label{tab:rq2}
    \centering
    \resizebox{0.6\textwidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Baby}} & \multicolumn{2}{c}{\textbf{Toys \& Games}} & \multicolumn{2}{c}{\textbf{Beauty}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        & Recall & nDCG & Recall & nDCG & Recall & nDCG \\ \cmidrule{1-7}
        \CC{20}BPRMF (\textsc{Base}) & \CC{20}4.56 & \CC{20}2.23 & \CC{20}8.55 & \CC{20}4.55 & \CC{20}9.43 & \CC{20}4.85 \\ \cmidrule{1-7}
        BPRMF-M (\textsc{Zeros}) & 5.03 & 2.49 & 10.07 & 5.42 & 9.80 & 5.08 \\
        BPRMF-M (\textsc{Random}) & 5.24 & 2.64 & 9.80 & 5.37 & 10.09 & 5.22 \\
        BPRMF-M (\textsc{GlobalMean}) & 4.98 & 2.46 & 9.76 & 5.33 & 10.55 & 5.55 \\
        \cmidrule{1-7}
        BPRMF-M (\textsc{NeighMean}) & 5.05 & 2.51 & 10.10 & 5.45 & 9.82 & 5.09 \\
        BPRMF-M (\textsc{PersPageRank}) \\
        BPRMF-M (\textsc{FeatProp}) & 5.71 & 2.82 & 10.37 & 5.62 & 10.83 & 5.73 \\
        \cmidrule{1-7} \textit{Improvement (\%)} \\
        \cmidrule{1-7} 
        \CC{20}NGCF (\textsc{Base}) & \CC{20}5.59 & \CC{20}2.81 & \CC{20}8.22 & \CC{20}4.23 & \CC{20}8.92 & \CC{20}4.56 \\ \cmidrule{1-7}
        NGCF-M (\textsc{Zeros}) & 6.76 & 3.39 & 8.56 & 4.38 & 9.64 & 4.99 \\
        NGCF-M (\textsc{Random}) & 6.57 & 3.30 & 8.32 & 4.31 & 9.74 & 5.01 \\
        NGCF-M (\textsc{GlobalMean}) & 6.89 & 3.50 & 8.62 & 4.39 & 9.73 & 5.02 \\
        \cmidrule{1-7}
        NGCF-M (\textsc{NeighMean}) & 7.00 & 3.57 & 8.77 & 4.48 & 10.32 & 5.35 \\
        NGCF-M (\textsc{PersPageRank}) & & &  &  \\
        NGCF-M (\textsc{FeatProp}) & 7.07 & 3.58 & inria & inria & cineca & cineca \\ \cmidrule{1-7} \textit{Improvement (\%)} \\
        \bottomrule
    \end{tabular}}
\end{table*}

==> tables/rq3_old_old.tex <==
\begin{table*}[!t]
\caption{}\label{tab:rq2}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcccccccccc}
    \toprule
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Digital Music}} & \multicolumn{2}{c}{\textbf{Office Products}} & \multicolumn{2}{c}{\textbf{Baby}} & \multicolumn{2}{c}{\textbf{Toys \& Games}} & \multicolumn{2}{c}{\textbf{Beauty}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        \cmidrule(lr){8-9}
        \cmidrule(lr){10-11}
        & Recall & nDCG & Recall & nDCG & Recall & nDCG & Recall & nDCG & Recall & nDCG \\ \cmidrule{1-11}
        \CC{20}BPRMF (\textsc{Base}) & \CC{20}24.59 & \CC{20}13.69 & \CC{20}8.51 & \CC{20}4.55 & \CC{20}4.56 & \CC{20}2.23 & \CC{20}8.55 & \CC{20}4.55 & \CC{20}9.43 & \CC{20}4.85 \\ \cmidrule{1-11}
        BPRMF-M (\textsc{Zeros}) & 24.85 & 14.02 & 9.49 & 5.24 & 5.03 & 2.49 & 10.07 & 5.42 & 9.80 & 5.08 \\
        BPRMF-M (\textsc{Random}) & 25.65 & 14.24 & 8.57 & 4.75 & 5.24 & 2.64 & 9.80 & 5.37 & 10.09 & 5.22 \\
        BPRMF-M (\textsc{GlobalMean}) & 24.81 & 14.03 & 9.46 & 5.30 & 4.98 & 2.46 & 9.76 & 5.33 & 10.55 & 5.55 \\
        \cmidrule{1-11}
        BPRMF-M (\textsc{NeighMean}) & 24.77 & 13.89 & 9.53 & 5.23 & 5.05 & 2.51 & 10.10 & 5.45 & 9.82 & 5.09 \\
        BPRMF-M (\textsc{PersPageRank}) \\
        BPRMF-M (\textsc{FeatProp}) & 26.03 & 14.56 & 10.09 & 5.41 & 5.71 & 2.82 & 10.37 & 5.62 & 10.83 & 5.73 \\
        \cmidrule{1-11} \textit{Improvement (\%)} &  &  &  &  &  &  &  &  \\
        \cmidrule{1-11} 
        \CC{20}NGCF (\textsc{Base}) & \CC{20}24.12 & \CC{20}13.06 & \CC{20}8.18 & \CC{20}3.91 & \CC{20}5.59 & \CC{20}2.81 & \CC{20}8.22 & \CC{20}4.23 & \CC{20}8.92 & \CC{20}4.56 \\ \cmidrule{1-11}
        NGCF-M (\textsc{Zeros}) & 24.14 & 13.03 & 10.55 & 5.34 & 6.76 & 3.39 & 8.56 & 4.38 & 9.64 & 4.99 \\
        NGCF-M (\textsc{Random}) & 24.42 & 13.28 & 10.44 & 5.19 & 6.57 & 3.30 & 8.32 & 4.31 & 9.74 & 5.01 \\
        NGCF-M (\textsc{GlobalMean}) & 23.99 & 13.05 & 10.69 & 5.35 & 6.89 & 3.50 & 8.62 & 4.39 & 9.73 & 5.02 \\
        \cmidrule{1-11}
        NGCF-M (\textsc{NeighMean}) & 23.86 & 12.65 & 11.33 & 5.79 & 7.00 & 3.57 & 8.77 & 4.48 & 10.32 & 5.35 \\
        NGCF-M (\textsc{PersPageRank}) & & &  &  \\
        NGCF-M (\textsc{FeatProp}) & 25.08 & 13.58 & 11.60 & 5.81 & 7.07 & 3.58 & inria & inria & cineca & cineca \\ \cmidrule{1-11} \textit{Improvement (\%)} \\\cmidrule{1-11} 
        \CC{20}LightGCN (\textsc{Base}) & \CC{20}26.61 & \CC{20}14.49 & \CC{20}11.55 & \CC{20}6.12 & \CC{20}7.36 & \CC{20}3.76 & \CC{20}10.22 & \CC{20}5.43 & \CC{20}11.61 & \CC{20}6.02 \\ \cmidrule{1-11}
        LightGCN-M (\textsc{Zeros}) & 26.75 & 14.59 & 11.69 & 6.40 & 7.71 & 3.89 & 10.44 & 5.60 & 12.02 & 6.33 \\
        LightGCN-M (\textsc{Random}) & 26.25 & 14.34 & 11.43 & 6.27 & 7.49 & 3.83 & 10.42 & 5.64 & 11.54 & 6.10\\
        LightGCN-M (\textsc{GlobalMean}) & 26.85 & 14.91 & 11.78 & 6.42 & 7.69 & 3.90 & 10.71 & 5.84 & 12.01 & 6.32 \\
        \cmidrule{1-11}
        LightGCN-M (\textsc{NeighMean}) & 27.37 & 15.21 &  12.01 & 6.69 & 7.74 & 3.92 & 11.26 & 6.06 & 12.03 & 6.32 \\
         LightGCN-M (\textsc{PersPageRank}) & & &  &  \\
        LightGCN-M (\textsc{FeatProp}) & 27.35 & 15.22 & 11.89 & 6.49 & 7.74 & 3.92 & 11.27 & 6.10 & 12.16 & 6.34 \\ \cmidrule{1-11} \textit{Improvement (\%)} \\
        \bottomrule
    \end{tabular}}
\end{table*}
